Towards Building Autonomous Data Services on Azure

Modern cloud has turned data services into easily accessible commodities. With just a few clicks, users are now able to access a catalog of data processing systems for a wide range of tasks. However, the cloud brings in both complexity and opportunity. While cloud users can quickly start an application by using various data services, it can be difficult to configure and optimize these services to gain the most value from them. For cloud providers, managing every aspect of an ever-increasing set of data services, while meeting customer SLAs and minimizing operational cost is becoming more challenging. Cloud technology enables the collection of significant amounts of workload traces and system telemetry. With the progress in data science (DS) and machine learning (ML), it is feasible and desirable to utilize a data-driven, ML-based approach to automate various aspects of data services, resulting in the creation of autonomous data services. This paper presents our perspectives and insights on creating autonomous data services on Azure. It also covers the future endeavors we plan to undertake and unresolved issues that still need attention.

==> old/insights_more.tex <==
% \subsection{Other challenges}
\begin{tcolorbox}[colback=black!5!white,colframe=black!80!white,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm}, left=0.1pt, right=0.1pt, arc=0pt,outer arc=0pt]
\myparr{Insight 4:} Sampling efficiency.
\end{tcolorbox}\vspace{-0.15cm}
As discussed in Section~\ref{sec:progress}, in many cases, collecting data for training ML models can be costly. When observational data is not sufficient, we can augment the training data by leveraging simulation~\cite{pimpley:tasq:edbt:2022, sen:autoexecutor:vldb:2021, sen:autoexecutor:edbt:2023}, or 
%conduct experiments to 
collect more data for the model to generalize better to the unseen scenarios. %Several techniques are used to help reduce the runs of experiment needed and improve the sampling efficient. 
Transfer learning~\cite{weiss2016survey} is commonly used in deep learning to use trained model as a warm-start, and similar approach can be applied, e.g., learning from benchmark workloads and transferring the learning to new customer workload. Dimension reduction~\cite{kanellis2022llamatune,ottertune} and tuning algorithms such as Bayesian optimization~\cite{bishop2006pattern} is also an option to improve the convergence speed to search for the optimal configuration setting.

\begin{tcolorbox}[colback=black!5!white,colframe=black!80!white,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm}, left=0.1pt, right=0.1pt, arc=0pt,outer arc=0pt]
\myparr{Insight 5:} Python for all?
%Even though Python is very popular, in many cases, it is not the optimal choice for productionized pipeline.
\end{tcolorbox}\vspace{-0.15cm}
We typically begin the majority of our DS engagements with Python, as it is convenient for visualization, data processing, model development and tuning.
% Python is our default language of choice for initial exploratory data analysis, for visualization and data processing, for model development and tuning. 
However, when it comes to integration with the rest of the infrastructure, 
% developing the E2E pipeline for production, 
Python is not always the default choice. This is particularly prominent in engagements in which the underlying production code is in another language where Python introduces latency and high overheads for maintenance and manageability. 
% [Maybe cite example from Deepak Ravikumar? the need to even change the model choice, python dependency issues] 
In some situations, we have to convert the Python code entirely to C\# for the production pipeline~\cite{doppler}. 
% This friction in language is one of the main obstacles we face in sharing infrastructure built in one service directly with another... but we overcome it [expand on Zendikon?] 
